Diversity Augmentation of Dynamic User Preference Data for Boosting Personalized Text Summarizers

Document summarization enables efficient extraction of user-relevant content but is inherently shaped by individual subjectivity, making it challenging to identify subjective salient information in multifaceted documents. This complexity underscores the necessity for personalized summarization. However, training models for personalized summarization has so far been challenging, particularly because diverse training data containing both user preference history (i.e., click-skip trajectory) and expected (gold-reference) summaries are scarce. The MS/CAS PENS dataset is a valuable resource but includes only preference history without target summaries, preventing end-to-end supervised learning, and its limited topic-transition diversity further restricts generalization. To address this, we propose $\mathrm{PerAugy}$, a novel cross-trajectory shuffling and summary-content perturbation based data augmentation technique that significantly boosts the accuracy of four state-of-the-art baseline (SOTA) user-encoders commonly used in personalized summarization frameworks (best result: $\text{0.132}$$\uparrow$ w.r.t AUC). We select two such SOTA summarizer frameworks as baselines and observe that when augmented with their corresponding improved user-encoders, they consistently show an increase in personalization (avg. boost: $\text{61.2\%}\uparrow$ w.r.t. PSE-SU4 metric). As a post-hoc analysis of the role of induced diversity in the augmented dataset by \peraugy, we introduce three dataset diversity metrics -- $\mathrm{TP}$, $\mathrm{RTC}$, and \degreed\ to quantify the induced diversity. We find that $\mathrm{TP}$ and $\mathrm{DegreeD}$ strongly correlate with user-encoder performance on the PerAugy-generated dataset across all accuracy metrics, indicating that increased dataset diversity is a key factor driving performance gains.

==> Additional/Ethics.tex <==
\section*{Ethics Statement}
We would like to declare that we used the PENS dataset and OpenAI (Reddit) dataset prepared and released by Microsoft Research/CAS and OpenAI respectively with complete compliance with the terms and conditions therein.

==> Main_Body/DegreeD.tex <==
\section{Measuring Preference Data Diversity}\label{sec:degreed}
To quantitatively measure the efficacy w.r.t diversity of any preference dataset (that can be modeled as a UIG), we propose a novel metric called \degreed\ (\textit{\textbf{Degree}-of-\textbf{D}iversity}) and then briefly discuss the method to compute it given any UIG.   

\subsection{\textbf{Degree}-of-\textbf{D}iversity (\degreed)}\label{sec:pens dataset diversity}
As a building block of the proposed metric \degreed, we first define \textit{\textbf{De}gree-of-\textbf{P}reference-\textbf{S}hift} (\deps) in a given UIG trajectory $\tau^{u_j}$ corresponding user $u_j$, where \deps\ quantifies the shift in a user's interest across $\tau^{u_j}$. 

\begin{definition}[\textbf{Degree of Preference Shift (\deps)}]\label{def:degree-of-preference-shift}
\deps\ is the ratio of the thematic divergence between consecutive d-nodes \( d^{(t_i)} \) and \( d^{(t_{i+1})} \) (denoted as \( \delta[X]_{d} \)) over a time span \(\Delta_{(t_i,t_{i+1})} = t_{i+1} - t_{i} \) and that between the corresponding s-nodes (user's subjective expected summaries) \( s_j^{(t_i)} \) and \( s_j^{(t_{i+1})} \) (denoted as \( \delta[X]_{s} \)).
\end{definition}
The thematic divergence $\delta[X]_{\bullet}$ ($\bullet \in \{d,s\}$) is calculated as $\sigma(\bullet^{t_i}_j,\bullet^{t_{i+1}}_j)$ where $\sigma$ is a distance measure on a chosen metric space. As per the definition, \deps\ for the $j$-th user at any unit interval $\Delta_{(t_i,t_{i+1})}$ is formulated as follows: 
\begin{equation}\label{eq:deps}
\begin{split}
        &\deps^{\Delta_{(t_i,t_{i+1})}}_{j} = \frac{min(\delta[X]_{d}, \delta[X]_{s_j})+\epsilon}{max(\delta[X]_{d}, \delta[X]_{s_j})+\epsilon}
        % & \delta[X]_{d_j} = \sigma(d^{t_i}_j,d^{t_{i+1}}_j); \ \ \delta[X]_{s_j} = \sigma(s^{t_i}_j,s^{t_{i+1}}_j) \\ & \Comment{\sigma: \text{distance measure on a chosen metric space}}
        % \frac{1}{|\profileset|} \sum\limits_{u=1}^{|\profileset|}
\end{split}
\end{equation}  
The Expected \deps, $\mathds{E}_j[\deps]$, for $j$-th user over the trajectory $\tau^{u_j}$ having length $l$ is:
\begin{equation}\label{eq:Expected Deps}
    \begin{split}
        & \mathds{E}_j[\deps] = \frac{1}{l-1} \sum\limits_{i=1}^{l-1} \deps^{\Delta_{(t_i,t_{i+1})}}_{j}
        % & \Comment{T: \text{Preference-trajectory length of user } j}
    \end{split}
\end{equation}
$\mathds{E}_j[\text{DePS}]$ penalizes the disproportionate alignment between the expected summaries ($\delta[X]_{s_j}$) and the document divergence ($\delta[X]_{d}$) for $\tau^{u_j}$ (Figure \ref{fig:degreed} (a)). However, it fails to penalize the case when any expected summary (s-node) in $\tau^{u_j}$ is not consistently faithful (in the sense of centrality to the core topic) to the corresponding document (d-node) (Figure \ref{fig:degreed} (b)). It also fails to penalize the case when the absolute thematic divergence is small (Figure \ref{fig:degreed} (c)). Both these cases can happen even with a high $\mathds{E}_j[\deps]$. To address the first issue, we modify $\mathds{E}_j[\deps]$ to incorporate the necessary penalties (i.e, penalized $\mathds{E}_j[\deps]$ or $\mathds{E}_j[\deps^\mathcal{P}]$) as follows:
\begin{equation}\label{eq:degreed}
    \begin{split}
        % & \degreed(\mathcal{D}) = \frac{\alpha}{|\profileset|}\cdot\sum_{j=1}^{|\profileset|} \delta[X]_{u_j}\cdot\mathds{E}_j[\deps^{\mathcal{P}}] \\ & \text{ where:}\\
        & \mathds{E}_j[\deps^{\mathcal{P}}] = \frac{\sum\limits_{i=1}^{l-1} \left(\deps^{\Delta_{(t_i,t_{i+1})}}_{j} \cdot \frac{\sigma(d^{(t_{i})},s^{(t_{i})}_j)}{\sigma(d^{(t_{i+1})},s^{(t_{i+1})}_j)}\right)}{l-1} 
    \end{split}
\end{equation}

\input{figures/fig:degreed penalties}

In the above equation, the second factor penalizes {\textit{negative shift}} in faithfulness where the s-node starts deviating away from the corresponding d-node as compared to the deviation at previous time-steps. Note that the \textbf{second factor rewards \textit{{positive shift}} where s-node comes closer to its corresponding d-node}. To address the second issue, we inject an additional factor $\delta[X]_{s_j}$ that penalizes lack of thematic divergence in terms of user's \underline{{actual interest/focus}} (hence, $\delta[X]_{s_j}$ instead of $\delta[X]_{d_j}$). $\delta[X]_{s_j}$ is regulated by the hyper-parameter $\alpha = (0,1]$. The final \degreed\ formulation for a UIG representing dataset $\mathcal{D}$ containing $|\mathbf{U}|$ unique user trajectories is:
\begin{equation}\label{eq:degreed}
    \begin{split}
        & \degreed(\mathcal{D}) = \frac{\alpha}{|\mathbf{U}|}\cdot\sum_{j=1}^{|\mathbf{U}|} \delta[X]_{s_j}\cdot\mathds{E}_j[\deps^{\mathcal{P}}] 
    \end{split}
\end{equation}
A dataset $\mathcal{D}$ is suitable for personalization training if it has a high \degreed\ score.

% \input{PseudoCodes/degreed_algo}

% \input{PseudoCodes/degreed_algo}
\subsection{\degreed\ Computation of UIGs}\label{sec:degreed computation}
In section \ref{sec:degreed}, we described a special case where for every d-node in an UIG we have a corresponding s-node in every trajectory $\tau$, which evidently is unrealistic. In reality, many of the d-nodes will not have a corresponding s-node and hence, the calculation of \deps\ cannot be done at every unit time-interval $\Delta_{(t_i,t_{i+1})}$. This requires modification in the computing procedure so as to account for the missing s-nodes. To address this, the first "\textit{surrogate}" s-node $s^{(t_1)}_j$ for the initial d-node $d^{(t_1)}$ at time-step $t_1$ is assumed to be the same as the document's title, as there is no prior preference history of a user at time-step $t_1$ and hence, subjectivity as a function of preference history does not arise yet. Let the first s-node $s^{(t_k)}_j$ occur at time-step $t_k$ (i.e., the first valid interval is $\Delta_{(t_1,t_k)}$). Therefore, $\deps^{\Delta_{(t_1,t_k)}}$ for $j$-th user is calculated as:  
\begin{equation}\label{eq:deps-computation}
\begin{split}
        &\deps^{\Delta_{(t_1,t_k)}}_{j} = \frac{min(\delta[X^{\Delta_{(t_1,t_k)}}]_{d}, \delta[X^{\Delta_{(t_1,t_k)}}]_{s_j})+\epsilon}{max(\delta[X^{\Delta_{(t_1,t_k)}}]_{d}, \delta[X^{\Delta_{(t_1,t_k)}}]_{s_j})+\epsilon};\\
        & \text{where: } \delta[X^{\Delta_{(t_1,t_k)}}]_{d} = \frac{1}{k-1}\cdot\sum_{i=1}^{k-1} \sigma(d^{(t_1)},d^{(t_{1+i})});  \delta[X^{\Delta_{(t_1,t_k)}}]_{s_j} = \sigma(s^{(t_1)}_j,s^{(t_{k})}_j) 
        % \\ & \Comment{\sigma: \text{distance measure on a chosen metric space}}
        % \frac{1}{|\profileset|} \sum\limits_{u=1}^{|\profileset|}
\end{split}
\end{equation}  
\degreed\ is then computed over all valid intervals as per equation \ref{eq:degreed}. In this paper, we represent d-nodes and s-nodes with their embeddings generated from a lightweight Sentence-BERT model (all-MiniLM-L6-v2) \cite{sbert-emnlp-2019} and use Manhattan Distance as the distance metric $\sigma$. In section \ref{sec:observations}, we empirically provide strong evidence that \text{higher UIG \degreed\ has strong correlation with user-encoder model accuracy} when trained on such UIGs (\degreed\ computation is in Algorithm \ref{algo:degreed-computation}).  We compute the \degreed\ of the PENS synthetic base pool $\mathcal{T}_{\text{base}}^{\text{syn-P}}$ and find a very low \degreed\ score of {\textcolor{black}{0.009}}. The OpenAI (Reddit) synthetic base pool $\mathcal{T}_{\text{base}}^{\text{syn-OAI}}$ also shows low \degreed\ of {\textcolor{black}{0.0079}}. In Section \ref{sec:observations}, we empirically show that \text{higher UIG \degreed\ has a strong correlation with user-encoder model accuracy} when trained on such UIGs\footnote{d/s-node embedding via SBERT model (all-MiniLM-L6-v2) \cite{sbert-emnlp-2019}; $\sigma:$ Manhattan distance}.

==> arxiv_preamble_fix.tex <==
% ===== arxiv_preamble_fix.tex (v2 minimal, collision-free) =====
% Put this right after \documentclass{...}

\RequirePackage{iftex}
\ifPDFTeX
  \RequirePackage[T1]{fontenc}
  \RequirePackage[utf8]{inputenc}
\else
  \RequirePackage{fontspec}
  \defaultfontfeatures{Ligatures=TeX}
  \setmainfont{Latin Modern Roman}
  \setsansfont{Latin Modern Sans}
  \setmonofont{Inconsolata}
\fi

% Micro-typography and colors
\RequirePackage{microtype}
\PassOptionsToPackage{dvipsnames,table}{xcolor}
\RequirePackage{xcolor}
\RequirePackage{colortbl}

% Map common Unicode punctuation so pdfLaTeX also survives.
\RequirePackage{newunicodechar}
\newunicodechar{’}{'}
\newunicodechar{‘}{`}
\newunicodechar{“}{``}
\newunicodechar{”}{''}
\newunicodechar{–}{--}
\newunicodechar{—}{---}
\newunicodechar{‑}{-}
\newunicodechar{‐}{-}

% Algorithmic stack — prefer algorithmicx + algpseudocode
\makeatletter
\let\AND\relax % avoid clashes with other packages
\makeatother
\RequirePackage{algorithm}
\RequirePackage{algorithmicx}
\RequirePackage{algpseudocode}
% Compatibility shim for older macros used in your pseudo-code files:
\providecommand{\RETURN}{\Return}

% Do NOT define \setuptodonotes here to avoid clashes.
% Instead, set the margin width right before loading todonotes in your main .tex:
% \setlength{\marginparwidth}{2.2c

==> figures/fig_degreed-comparison.tex <==
% \begin{figure*}[h]
% \includegraphics[width=\textwidth,keepaspectratio,trim={0 0 0 0},clip]{figures/fig:degreed comparisons.pdf}
% \caption{Caption - to be updated by Amey}
% \label{fig:degreed-comparative study}
% % \vspace{-0.25mm}
% \vspace{-5mm}
% \end{figure*}

==> figures/fig_peraugy_main_results.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]
%,keepaspectratio,trim={0 0 0 0},clip]
{figures/peraugy_figure4_updated3.pdf}
\caption{\textbf{PerAugy Performance (Summary)}: (a) Increase in DegreeD in comparison to baseline augmentation methods w.r.t SMP hyper-parameters (context-window $k$, decay constant $\lambda$, perturbation probability $p_{\text{SMP}}$), (b) Average increase in accuracy of user-encoders, \& (c) Best PSE-SU4 performances of personalized summarizers w.r.t \textit{\colorbox{lightteal}{original}}, \textit{\colorbox{yellow}{train-from-scratch}}, and \textit{\colorbox{orange}{fine-tuned}} user-encoders injections. Detailed results in Appendix \ref{app:detailed results}.}
\label{fig:peraugy_performance}
\vspace{-4.5mm}
\end{figure*}

==> figures/figure5.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth,keepaspectratio,trim={0 0 0 0},clip]{figures/peraugy_figure5.pdf}
\caption{Caption - To be updated by Amey}
\label{fig:figure5}
% \vspace{-0.25mm}
\vspace{-5mm}
\end{figure*}

==> tables/tab_degreed-ablations.tex <==
% Ablation DegreeD results
\begin{table*}[t]
\centering  
\scalebox{0.5}
{
    \begin{tabular}{ccccccccccccccccccc}
        \cmidrule(lr){1-5} \cmidrule(lr){6-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
        \multicolumn{5}{c}{\textbf{DS: Gap Length ($g_l$)}} & \multicolumn{5}{c}{\textbf{DS: Trajectory Length ($l$)}} & \multicolumn{3}{c}{\textbf{SMP: Context-Window ($k$)}} & \multicolumn{3}{c}{\textbf{SMP: Decay Constant ($\lambda$)}} & \multicolumn{3}{c}{\textbf{SMP: Perturbation Probability ($p_{\text{SMP}}$)}} \\
        \cmidrule(lr){1-5} \cmidrule(lr){6-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
        \multicolumn{1}{c}{\textbf{10}} & \multicolumn{1}{c}{15} & \multicolumn{1}{c}{20} & \multicolumn{1}{c}{25} & \multicolumn{1}{c}{40} & \multicolumn{1}{c}{50} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{125} & \multicolumn{1}{c}{\textbf{175}} & \multicolumn{1}{c}{200} & \multicolumn{1}{c}{\textbf{10}} & \multicolumn{1}{c}{15} & \multicolumn{1}{c}{20} & \multicolumn{1}{c}{\textbf{0.3}} & \multicolumn{1}{c}{0.8} & \multicolumn{1}{c}{1.0} & \multicolumn{1}{c}{0.5} & \multicolumn{1}{c}{0.8} & \multicolumn{1}{c}{\textbf{1.0}} \\
        \cmidrule(lr){1-5} \cmidrule(lr){6-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
        \multicolumn{1}{c}{\textbf{0.163}} & \multicolumn{1}{c}{0.146} & \multicolumn{1}{c}{0.134} & \multicolumn{1}{c}{0.137} & \multicolumn{1}{c}{0.127} & \multicolumn{1}{c}{0.133} & \multicolumn{1}{c}{0.138} & \multicolumn{1}{c}{0.143} & \multicolumn{1}{c}{\textbf{0.158}} & \multicolumn{1}{c}{0.148} & \multicolumn{1}{c}{\textbf{0.273}} & \multicolumn{1}{c}{0.256} & \multicolumn{1}{c}{0.243} & \multicolumn{1}{c}{\textbf{0.271}} & \multicolumn{1}{c}{0.209} & \multicolumn{1}{c}{0.184} & \multicolumn{1}{c}{0.237} & \multicolumn{1}{c}{0.274} & \multicolumn{1}{c}{\textbf{0.277}} \\
        \cmidrule(lr){1-5} \cmidrule(lr){6-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
        % \hline
    \end{tabular}
}
\caption{\textbf{Ablation (RQ-1) Effect of Hyper-parameters on \degreed:} Diversity analysis for all hyper-parameters of \peraugy; \textbf{Observation-1}: \textit{lower gap length increases diversity due to diffusion into different topics across a trajectory}; \textbf{Observation-2}: \textit{Longer context window may not lead to sufficient perturbation}; \textbf{Observation-3}: \textit{stricter Markovian does not yield higher diversity}; \& \textbf{Observation 4}: \textit{frequent SMP ops. on s-nodes lead to higher diversity}.}
\label{tab:ablation-degreed}
% \vspace{-8mm}
\end{table*}


% \begin{table*}[!ht]
% \begin{center}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccccccccc}
% \toprule
% \textbf{Hyper-parameters} & \multicolumn{4}{c}{\textbf{NAML}} & \multicolumn{4}{c}{\textbf{EBNR}} & \multicolumn{4}{c}{\textbf{NRMS}} & \multicolumn{4}{c}{\textbf{TrRMIo w/ Title}} \\ 
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
% & AUC & MRR & NDCG@5 & NDCG@10 & AUC & MRR & NDCG@5 & NDCG@10 & AUC & MRR & NDCG@5 & NDCG@10 & AUC & MRR & NDCG@5 & NDCG@10 \\ 
% \midrule

% \multicolumn{17}{c}{\textbf{Ablation DS-History (trajectory-length = 150)}} \\
% \midrule
% DS: G=10 & \cellcolor{ForestGreen!50}0.5436 & \cellcolor{ForestGreen!60}0.7718 & \cellcolor{ForestGreen!70}0.8315 & \cellcolor{ForestGreen!70}0.8315 & \cellcolor{ForestGreen!40}0.5825 & \cellcolor{ForestGreen!65}0.7912 & \cellcolor{ForestGreen!75}0.8459 & \cellcolor{ForestGreen!75}0.8459 & \cellcolor{ForestGreen!40}0.5825 & \cellcolor{ForestGreen!65}0.7912 & \cellcolor{ForestGreen!75}0.8459 & \cellcolor{ForestGreen!75}0.8459 & \cellcolor{ForestGreen!50}0.5448 & \cellcolor{ForestGreen!55}0.7168 & \cellcolor{ForestGreen!65}0.7934 & \cellcolor{ForestGreen!65}0.7934 \\
% DS: G=15 & \cellcolor{ForestGreen!50}0.5436 & \cellcolor{ForestGreen!60}0.7718 & \cellcolor{ForestGreen!70}0.8315 & \cellcolor{ForestGreen!70}0.8315 & \cellcolor{ForestGreen!45}0.6116 & \cellcolor{ForestGreen!67}0.8058 & \cellcolor{ForestGreen!77}0.8566 & \cellcolor{ForestGreen!77}0.8566 & \cellcolor{ForestGreen!50}0.5436 & \cellcolor{ForestGreen!60}0.7718 & \cellcolor{ForestGreen!70}0.8315 & \cellcolor{ForestGreen!70}0.8315 & \cellcolor{ForestGreen!45}0.5419 & \cellcolor{ForestGreen!50}0.7043 & \cellcolor{ForestGreen!60}0.7815 & \cellcolor{ForestGreen!60}0.7815 \\
% DS: G=20 & \cellcolor{ForestGreen!55}0.5631 & \cellcolor{ForestGreen!62}0.7815 & \cellcolor{ForestGreen!72}0.8387 & \cellcolor{ForestGreen!72}0.8387 & \cellcolor{ForestGreen!50}0.5533 & \cellcolor{ForestGreen!64}0.7766 & \cellcolor{ForestGreen!74}0.8351 & \cellcolor{ForestGreen!74}0.8351 & \cellcolor{ForestGreen!40}0.5145 & \cellcolor{ForestGreen!60}0.7572 & \cellcolor{ForestGreen!70}0.8208 & \cellcolor{ForestGreen!70}0.8208 & \cellcolor{ForestGreen!50}0.5518 & \cellcolor{ForestGreen!55}0.7212 & \cellcolor{ForestGreen!65}0.7975 & \cellcolor{ForestGreen!65}0.7975 \\
% DS: G=25 & \cellcolor{ForestGreen!55}0.5533 & \cellcolor{ForestGreen!62}0.7766 & \cellcolor{ForestGreen!72}0.8315 & \cellcolor{ForestGreen!72}0.8315 & \cellcolor{ForestGreen!50}0.5631 & \cellcolor{ForestGreen!64}0.7815 & \cellcolor{ForestGreen!74}0.8387 & \cellcolor{ForestGreen!74}0.8387 & \cellcolor{ForestGreen!40}0.5436 & \cellcolor{ForestGreen!60}0.7718 & \cellcolor{ForestGreen!70}0.8315 & \cellcolor{ForestGreen!70}0.8315 & \cellcolor{ForestGreen!50}0.5583 & \cellcolor{ForestGreen!55}0.7245 & \cellcolor{ForestGreen!65}0.7993 & \cellcolor{ForestGreen!65}0.7993 \\
% DS: G=40 & \cellcolor{ForestGreen!55}0.5631 & \cellcolor{ForestGreen!62}0.7815 & \cellcolor{ForestGreen!72}0.8387 & \cellcolor{ForestGreen!72}0.8387 & \cellcolor{ForestGreen!50}0.6019 & \cellcolor{ForestGreen!64}0.8009 & \cellcolor{ForestGreen!74}0.8530 & \cellcolor{ForestGreen!74}0.8530 & \cellcolor{ForestGreen!40}0.5145 & \cellcolor{ForestGreen!60}0.7572 & \cellcolor{ForestGreen!70}0.8208 & \cellcolor{ForestGreen!70}0.8208 & \cellcolor{ForestGreen!50}0.5319 & \cellcolor{ForestGreen!55}0.7043 & \cellcolor{ForestGreen!65}0.7618 & \cellcolor{ForestGreen!65}0.7618 \\
% \midrule
% \multicolumn{17}{c}{\textbf{Ablation DS-History (Gap = 25)}} \\
% \midrule
% DS: $l/2$ & \cellcolor{ForestGreen!45}0.6116 & \cellcolor{ForestGreen!67}0.8058 & \cellcolor{ForestGreen!77}0.8566 & \cellcolor{ForestGreen!77}0.8566 & \cellcolor{ForestGreen!35}0.5339 & \cellcolor{ForestGreen!62}0.7669 & \cellcolor{ForestGreen!72}0.8280 & \cellcolor{ForestGreen!72}0.8280 & \cellcolor{ForestGreen!55}0.5631 & \cellcolor{ForestGreen!62}0.7815 & \cellcolor{ForestGreen!72}0.8387 & \cellcolor{ForestGreen!72}0.8387 & \cellcolor{ForestGreen!40}0.5314 & \cellcolor{ForestGreen!50}0.7527 & \cellcolor{ForestGreen!65}0.8013 & \cellcolor{ForestGreen!65}0.8013 \\
% DS: $5/8*l$ & \cellcolor{ForestGreen!55}0.5631 & \cellcolor{ForestGreen!62}0.7815 & \cellcolor{ForestGreen!72}0.8387 & \cellcolor{ForestGreen!72}0.8387 & \cellcolor{ForestGreen!30}0.4951 & \cellcolor{ForestGreen!57}0.7475 & \cellcolor{ForestGreen!67}0.8136 & \cellcolor{ForestGreen!67}0.8136 & \cellcolor{ForestGreen!45}0.5242 & \cellcolor{ForestGreen!62}0.7621 & \cellcolor{ForestGreen!72}0.8244 & \cellcolor{ForestGreen!72}0.8244 & \cellcolor{ForestGreen!50}0.5517 & \cellcolor{ForestGreen!67}0.7683 & \cellcolor{ForestGreen!72}0.8135 & \cellcolor{ForestGreen!72}0.8135 \\
% DS: $3/4*l$ & \cellcolor{ForestGreen!55}0.5922 & \cellcolor{ForestGreen!62}0.7961 & \cellcolor{ForestGreen!72}0.8495 & \cellcolor{ForestGreen!72}0.8495 & \cellcolor{ForestGreen!30}0.5533 & \cellcolor{ForestGreen!57}0.7766 & \cellcolor{ForestGreen!67}0.8351 & \cellcolor{ForestGreen!67}0.8351 & \cellcolor{ForestGreen!45}0.5145 & \cellcolor{ForestGreen!62}0.7572 & \cellcolor{ForestGreen!72}0.8208 & \cellcolor{ForestGreen!72}0.8208 & \cellcolor{ForestGreen!50}0.5319 & \cellcolor{ForestGreen!67}0.7314 & \cellcolor{ForestGreen!72}0.7937 & \cellcolor{ForestGreen!72}0.7937 \\
% DS: $7/8*l$ & \cellcolor{ForestGreen!55}0.5922 & \cellcolor{ForestGreen!62}0.7961 & \cellcolor{ForestGreen!72}0.8495 & \cellcolor{ForestGreen!72}0.8495 & \cellcolor{ForestGreen!30}0.5436 & \cellcolor{ForestGreen!57}0.7718 & \cellcolor{ForestGreen!67}0.8315 & \cellcolor{ForestGreen!67}0.8315 & \cellcolor{ForestGreen!45}0.5145 & \cellcolor{ForestGreen!62}0.7572 & \cellcolor{ForestGreen!72}0.8208 & \cellcolor{ForestGreen!72}0.8208 & \cellcolor{ForestGreen!50}0.5618 & \cellcolor{ForestGreen!67}0.7419 & \cellcolor{ForestGreen!72}0.7914 & \cellcolor{ForestGreen!72}0.7914 \\
% DS: $l-3$ & \cellcolor{ForestGreen!55}0.6019 & \cellcolor{ForestGreen!62}0.8009 & \cellcolor{ForestGreen!72}0.8530 & \cellcolor{ForestGreen!72}0.8530 & \cellcolor{ForestGreen!30}0.5728 & \cellcolor{ForestGreen!57}0.7864 & \cellcolor{ForestGreen!67}0.8423 & \cellcolor{ForestGreen!67}0.8423 & \cellcolor{ForestGreen!45}0.4951 & \cellcolor{ForestGreen!62}0.7475 & \cellcolor{ForestGreen!72}0.8136 & \cellcolor{ForestGreen!72}0.8136 & \cellcolor{ForestGreen!50}0.5915 & \cellcolor{ForestGreen!67}0.7758 & \cellcolor{ForestGreen!72}0.8311 & \cellcolor{ForestGreen!72}0.8311 \\
% \midrule
% % ===========================================================================================
% \multicolumn{17}{c}{\textbf{Ablation SMP-k (Context Window; \(\lambda\) = 0.5; $P_{\text{SMP}}$ = 0.8)}} \\
% \midrule
% SMP: k=10 & \cellcolor{ForestGreen!40}0.6431 & \cellcolor{ForestGreen!60}0.8345 & \cellcolor{ForestGreen!70}0.8912 & \cellcolor{ForestGreen!70}0.8912 & \cellcolor{ForestGreen!50}0.6186 & \cellcolor{ForestGreen!62}0.7818 & \cellcolor{ForestGreen!67}0.8515 & \cellcolor{ForestGreen!67}0.8512 & \cellcolor{ForestGreen!55}0.6381 & \cellcolor{ForestGreen!67}0.8122 & \cellcolor{ForestGreen!75}0.8768 & \cellcolor{ForestGreen!75}0.8768 & \cellcolor{ForestGreen!55}0.5618 & \cellcolor{ForestGreen!50}0.7438 & \cellcolor{ForestGreen!60}0.8247 & \cellcolor{ForestGreen!60}0.8247 \\
% SMP: k=15 & \cellcolor{ForestGreen!40}0.6511 & \cellcolor{ForestGreen!60}0.8091 & \cellcolor{ForestGreen!70}0.8871 & \cellcolor{ForestGreen!70}0.8871 & \cellcolor{ForestGreen!50}0.6356 & \cellcolor{ForestGreen!62}0.7934 & \cellcolor{ForestGreen!67}0.8411 & \cellcolor{ForestGreen!67}0.8411 & \cellcolor{ForestGreen!55}0.5713 & \cellcolor{ForestGreen!67}0.7924 & \cellcolor{ForestGreen!75}0.8411 & \cellcolor{ForestGreen!75}0.8411 & \cellcolor{ForestGreen!55}0.5413 & \cellcolor{ForestGreen!50}0.7319 & \cellcolor{ForestGreen!60}0.8091 & \cellcolor{ForestGreen!60}0.8091 \\
% SMP: k=20 & \cellcolor{ForestGreen!40}0.6356 & \cellcolor{ForestGreen!60}0.8123 & \cellcolor{ForestGreen!70}0.8896 & \cellcolor{ForestGreen!70}0.8896 & \cellcolor{ForestGreen!50}0.5984 & \cellcolor{ForestGreen!62}0.7632 & \cellcolor{ForestGreen!67}0.8187 & \cellcolor{ForestGreen!67}0.8187 & \cellcolor{ForestGreen!55}0.5267 & \cellcolor{ForestGreen!67}0.7892 & \cellcolor{ForestGreen!75}0.8403 & \cellcolor{ForestGreen!75}0.8403 & \cellcolor{ForestGreen!55}0.5315 & \cellcolor{ForestGreen!50}0.7148 & \cellcolor{ForestGreen!60}0.7713 & \cellcolor{ForestGreen!60}0.7713 \\
% \midrule
% % ===========================================================================================
% \multicolumn{17}{c}{\textbf{Ablation SMP-\(\lambda\) (Decay Factor; k=10; $P_{\text{SMP}}$ = 0.8)}} \\
% \midrule
% \(\lambda\) = 0.3 & \cellcolor{ForestGreen!40}0.6018 & \cellcolor{ForestGreen!60}0.7816 & \cellcolor{ForestGreen!70}0.8248 & \cellcolor{ForestGreen!70}0.8248 & \cellcolor{ForestGreen!50}0.6518 & \cellcolor{ForestGreen!62}0.7858 & \cellcolor{ForestGreen!67}0.8617 & \cellcolor{ForestGreen!67}0.8617 & \cellcolor{ForestGreen!55}0.5412 & \cellcolor{ForestGreen!67}0.7491 & \cellcolor{ForestGreen!75}0.7932 & \cellcolor{ForestGreen!75}0.7932 & \cellcolor{ForestGreen!55}0.5614 & \cellcolor{ForestGreen!50}0.7346 & \cellcolor{ForestGreen!60}0.7821 & \cellcolor{ForestGreen!60}0.7821 \\
% \(\lambda\) = 0.8 & \cellcolor{ForestGreen!40}0.6076 & \cellcolor{ForestGreen!60}0.7582 & \cellcolor{ForestGreen!70}0.8114 & \cellcolor{ForestGreen!70}0.8114 & \cellcolor{ForestGreen!50}0.5942 & \cellcolor{ForestGreen!62}0.7319 & \cellcolor{ForestGreen!67}0.8312 & \cellcolor{ForestGreen!67}0.8312 & \cellcolor{ForestGreen!55}0.5388 & \cellcolor{ForestGreen!67}0.7245 & \cellcolor{ForestGreen!75}0.7839 & \cellcolor{ForestGreen!75}0.7839 & \cellcolor{ForestGreen!55}0.5517 & \cellcolor{ForestGreen!50}0.7422 & \cellcolor{ForestGreen!60}0.7807 & \cellcolor{ForestGreen!60}0.7807 \\
% \(\lambda\) = 1.0 & \cellcolor{ForestGreen!40}0.5812 & \cellcolor{ForestGreen!60}0.7219 & \cellcolor{ForestGreen!70}0.7927 & \cellcolor{ForestGreen!70}0.7927 & \cellcolor{ForestGreen!50}0.5930 & \cellcolor{ForestGreen!62}0.7488 & \cellcolor{ForestGreen!67}0.8475 & \cellcolor{ForestGreen!67}0.8475 & \cellcolor{ForestGreen!55}0.5281 & \cellcolor{ForestGreen!67}0.7162 & \cellcolor{ForestGreen!75}0.7715 & \cellcolor{ForestGreen!75}0.7715 & \cellcolor{ForestGreen!55}0.5218 & \cellcolor{ForestGreen!50}0.6993 & \cellcolor{ForestGreen!60}0.7519 & \cellcolor{ForestGreen!60}0.7519 \\
% \midrule
% % =============================================================================================
% \multicolumn{17}{c}{\textbf{Ablation SMP-Probability ($P_{\text{SMP}}$; k=10; \(\lambda\) = 0.5)}} \\
% \midrule
% $P_{\text{SMP}}$ = 0.5 & \cellcolor{ForestGreen!40}0.5337 & \cellcolor{ForestGreen!60}0.7718 & \cellcolor{ForestGreen!70}0.8419 & \cellcolor{ForestGreen!70}0.8419 & \cellcolor{ForestGreen!50}0.5918 & \cellcolor{ForestGreen!62}0.7683 & \cellcolor{ForestGreen!67}0.8201 & \cellcolor{ForestGreen!67}0.8201 & \cellcolor{ForestGreen!55}0.5782 & \cellcolor{ForestGreen!67}0.7765 & \cellcolor{ForestGreen!75}0.8445 & \cellcolor{ForestGreen!75}0.8445 & \cellcolor{ForestGreen!55}0.5783 & \cellcolor{ForestGreen!50}0.7311 & \cellcolor{ForestGreen!60}0.7834 & \cellcolor{ForestGreen!60}0.7834 \\
% $P_{\text{SMP}}$ = 0.8 & \cellcolor{ForestGreen!40}0.5791 & \cellcolor{ForestGreen!60}0.7923 & \cellcolor{ForestGreen!70}0.8634 & \cellcolor{ForestGreen!70}0.8634 & \cellcolor{ForestGreen!50}0.6175 & \cellcolor{ForestGreen!62}0.7864 & \cellcolor{ForestGreen!67}0.8596 & \cellcolor{ForestGreen!67}0.8596 & \cellcolor{ForestGreen!55}0.5937 & \cellcolor{ForestGreen!67}0.7845 & \cellcolor{ForestGreen!75}0.8519 & \cellcolor{ForestGreen!75}0.8519 & \cellcolor{ForestGreen!55}0.5854 & \cellcolor{ForestGreen!50}0.7691 & \cellcolor{ForestGreen!60}0.8281 & \cellcolor{ForestGreen!60}0.8281 \\
% $P_{\text{SMP}}$ = 1.0 & \cellcolor{ForestGreen!40}0.5874 & \cellcolor{ForestGreen!60}0.8145 & \cellcolor{ForestGreen!70}0.8828 & \cellcolor{ForestGreen!70}0.8828 & \cellcolor{ForestGreen!50}0.5685 & \cellcolor{ForestGreen!62}0.7538 & \cellcolor{ForestGreen!67}0.8398 & \cellcolor{ForestGreen!67}0.8398 & \cellcolor{ForestGreen!55}0.5725 & \cellcolor{ForestGreen!67}0.7649 & \cellcolor{ForestGreen!75}0.8431 & \cellcolor{ForestGreen!75}0.8431 & \cellcolor{ForestGreen!55}0.6137 & \cellcolor{ForestGreen!50}0.7913 & \cellcolor{ForestGreen!60}0.8522 & \cellcolor{ForestGreen!60}0.8522 \\
% \bottomrule
% \end{tabular}%
% }
% \end{center}
% \caption{Amey - The heatmap (color grading) values are not properly set yet. This would be a manual thing, so keeping it at last. }
% \vspace{-3mm}
% \label{tab:ablations-accuracy}
% \end{table*}




==> tables/tab_encoder-ablations.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccc}
\toprule
\multirow{2}{*}{\makecell{\textbf{Hyper-} \\ \textbf{parameters}}}  & \multicolumn{4}{c}{\textbf{NAML}} 
  & \multicolumn{4}{c}{\textbf{EBNR}} 
  & \multicolumn{4}{c}{\textbf{NRMS}} 
  & \multicolumn{4}{c}{\makecell{\textbf{TrRMIo} \\ \textbf{w/ Title}}} \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
  & AUC & MRR & NDCG@5 & NDCG@10 
  & AUC & MRR & NDCG@5 & NDCG@10 
  & AUC & MRR & NDCG@5 & NDCG@10 
  & AUC & MRR & NDCG@5 & NDCG@10 \\ 
\midrule

\multicolumn{17}{c}{\makecell{\textbf{DS: Gap-Length ($g_l$)} \\ \textbf{(fixed trajectory-length = 150)}}} \\
\midrule
10 
  & \cellcolor{white!20}0.54 & \cellcolor{white!35}0.77 & \cellcolor{white!50}0.83 & \cellcolor{white!50}0.83 
  & \cellcolor{white!25}0.58 & \cellcolor{white!40}0.79 & \cellcolor{white!60}0.85 & \cellcolor{white!60}0.85 
  & \cellcolor{white!25}0.58 & \cellcolor{white!40}0.79 & \cellcolor{white!60}0.85 & \cellcolor{white!60}0.85 
  & \cellcolor{white!20}0.54 & \cellcolor{white!30}0.72 & \cellcolor{white!45}0.79 & \cellcolor{white!45}0.79 \\

\textbf{15} 
  & \cellcolor{white!20}0.54 & \cellcolor{white!35}0.77 & \cellcolor{white!50}0.83 & \cellcolor{white!50}0.83 
  & \cellcolor{white!35}\textbf{0.61} & \cellcolor{white!50}\textbf{0.81} & \cellcolor{white!65}\textbf{0.86} & \cellcolor{white!65}\textbf{0.86} 
  & \cellcolor{white!20}0.54 & \cellcolor{white!35}0.77 & \cellcolor{white!50}0.83 & \cellcolor{white!50}0.83 
  & \cellcolor{white!15}0.54 & \cellcolor{white!25}0.7  & \cellcolor{white!40}0.78 & \cellcolor{white!40}0.78 \\

20 
  & \cellcolor{white!30}\textbf{0.56} & \cellcolor{white!40}\textbf{0.78} & \cellcolor{white!55}\textbf{0.84} & \cellcolor{white!55}\textbf{0.84} 
  & \cellcolor{white!30}0.55 & \cellcolor{white!42}0.78 & \cellcolor{white!58}0.84 & \cellcolor{white!58}0.84 
  & \cellcolor{white!15}0.51 & \cellcolor{white!30}0.76 & \cellcolor{white!50}0.82 & \cellcolor{white!50}0.82 
  & \cellcolor{white!20}0.55 & \cellcolor{white!28}0.72 & \cellcolor{white!42}0.8  & \cellcolor{white!42}0.8  \\

25 
  & \cellcolor{white!30}0.55 & \cellcolor{white!40}0.78 & \cellcolor{white!55}0.83 & \cellcolor{white!55}0.83 
  & \cellcolor{white!30}\textbf{0.56} & \cellcolor{white!42}\textbf{0.78} & \cellcolor{white!58}\textbf{0.84} & \cellcolor{white!58}\textbf{0.84} 
  & \cellcolor{white!20}0.54 & \cellcolor{white!35}0.77 & \cellcolor{white!50}0.83 & \cellcolor{white!50}0.83 
  & \cellcolor{white!22}0.56 & \cellcolor{white!28}0.72 & \cellcolor{white!42}0.8  & \cellcolor{white!42}0.8  \\

40 
  & \cellcolor{white!35}0.56 & \cellcolor{white!45}0.78 & \cellcolor{white!60}0.84 & \cellcolor{white!60}0.84 
  & \cellcolor{white!40}\textbf{0.6}  & \cellcolor{white!50}\textbf{0.8}  & \cellcolor{white!65}\textbf{0.85} & \cellcolor{white!65}\textbf{0.85} 
  & \cellcolor{white!15}0.51 & \cellcolor{white!30}0.76 & \cellcolor{white!50}0.82 & \cellcolor{white!50}0.82 
  & \cellcolor{white!15}0.53 & \cellcolor{white!25}0.7  & \cellcolor{white!38}0.76 & \cellcolor{white!38}0.76 \\

\midrule
\multicolumn{17}{c}{\makecell{\textbf{DS: History ($\tau_{h_{\text{train}}}$)}\\ \textbf{(fixed gap = 25)}}} \\
\midrule
\textbf{$l/2$} 
  & \cellcolor{white!40}\textbf{0.61} & \cellcolor{white!55}\textbf{0.81} & \cellcolor{white!65}\textbf{0.86} & \cellcolor{white!65}\textbf{0.86} 
  & \cellcolor{white!25}0.53 & \cellcolor{white!42}0.77 & \cellcolor{white!58}0.83 & \cellcolor{white!58}0.83 
  & \cellcolor{white!35}0.56 & \cellcolor{white!45}0.78 & \cellcolor{white!60}0.84 & \cellcolor{white!60}0.84 
  & \cellcolor{white!30}0.53 & \cellcolor{white!38}0.75 & \cellcolor{white!50}0.8  & \cellcolor{white!50}0.8  \\

$5/8*l$ 
  & \cellcolor{white!30}\textbf{0.56} & \cellcolor{white!45}\textbf{0.78} & \cellcolor{white!60}\textbf{0.84} & \cellcolor{white!60}\textbf{0.84} 
  & \cellcolor{white!20}0.5  & \cellcolor{white!38}0.75 & \cellcolor{white!55}0.81 & \cellcolor{white!55}0.81 
  & \cellcolor{white!30}0.52 & \cellcolor{white!45}0.76 & \cellcolor{white!60}0.82 & \cellcolor{white!60}0.82 
  & \cellcolor{white!35}0.55 & \cellcolor{white!50}0.77 & \cellcolor{white!60}0.81 & \cellcolor{white!60}0.81 \\

$3/4*l$ 
  & \cellcolor{white!35}\textbf{0.59} & \cellcolor{white!50}\textbf{0.8}  & \cellcolor{white!62}\textbf{0.85} & \cellcolor{white!62}\textbf{0.85} 
  & \cellcolor{white!25}0.55 & \cellcolor{white!40}0.78 & \cellcolor{white!58}0.84 & \cellcolor{white!58}0.84 
  & \cellcolor{white!28}0.51 & \cellcolor{white!42}0.76 & \cellcolor{white!58}0.82 & \cellcolor{white!58}0.82 
  & \cellcolor{white!30}0.53 & \cellcolor{white!42}0.73 & \cellcolor{white!55}0.79 & \cellcolor{white!55}0.79 \\

$7/8*l$ 
  & \cellcolor{white!35}\textbf{0.59} & \cellcolor{white!50}\textbf{0.8}  & \cellcolor{white!62}\textbf{0.85} & \cellcolor{white!62}\textbf{0.85} 
  & \cellcolor{white!22}0.54 & \cellcolor{white!38}0.77 & \cellcolor{white!55}0.83 & \cellcolor{white!55}0.83 
  & \cellcolor{white!28}0.51 & \cellcolor{white!42}0.76 & \cellcolor{white!58}0.82 & \cellcolor{white!58}0.82 
  & \cellcolor{white!32}0.56 & \cellcolor{white!44}0.74 & \cellcolor{white!55}0.79 & \cellcolor{white!55}0.79 \\

$l-3$ 
  & \cellcolor{white!40}\textbf{0.6}  & \cellcolor{white!55}\textbf{0.8}  & \cellcolor{white!65}\textbf{0.85} & \cellcolor{white!65}\textbf{0.85} 
  & \cellcolor{white!28}0.57 & \cellcolor{white!42}0.79 & \cellcolor{white!60}0.84 & \cellcolor{white!60}0.84 
  & \cellcolor{white!25}0.5  & \cellcolor{white!40}0.75 & \cellcolor{white!55}0.81 & \cellcolor{white!55}0.81 
  & \cellcolor{white!35}0.59 & \cellcolor{white!50}0.78 & \cellcolor{white!60}0.83 & \cellcolor{white!60}0.83 \\

\midrule
\multicolumn{17}{c}{\makecell{\textbf{SMP: Context Window ($k$)} \\\textbf{(fixed \(\lambda\)=0.5; $P_{\text{SMP}}$=0.8)}}} \\
\midrule
10 
  & \cellcolor{white!45}\textbf{0.64} & \cellcolor{white!65}\textbf{0.83} & \cellcolor{white!75}\textbf{0.89} & \cellcolor{white!75}\textbf{0.89} 
  & \cellcolor{white!40}0.62 & \cellcolor{white!50}0.78 & \cellcolor{white!60}0.85 & \cellcolor{white!60}0.85 
  & \cellcolor{white!50}0.64 & \cellcolor{white!58}0.81 & \cellcolor{white!68}0.88 & \cellcolor{white!68}0.88 
  & \cellcolor{white!38}0.56 & \cellcolor{white!42}0.74 & \cellcolor{white!52}0.82 & \cellcolor{white!52}0.82 \\

\textbf{15} 
  & \cellcolor{white!48}\textbf{0.65} & \cellcolor{white!63}\textbf{0.81} & \cellcolor{white!72}\textbf{0.89} & \cellcolor{white!72}\textbf{0.89} 
  & \cellcolor{white!42}0.64 & \cellcolor{white!53}0.79 & \cellcolor{white!63}0.84 & \cellcolor{white!63}0.84 
  & \cellcolor{white!45}0.57 & \cellcolor{white!58}0.79 & \cellcolor{white!68}0.84 & \cellcolor{white!68}0.84 
  & \cellcolor{white!35}0.54 & \cellcolor{white!40}0.73 & \cellcolor{white!50}0.81 & \cellcolor{white!50}0.81 \\

20 
  & \cellcolor{white!42}\textbf{0.64} & \cellcolor{white!60}\textbf{0.81} & \cellcolor{white!70}\textbf{0.89} & \cellcolor{white!70}\textbf{0.89} 
  & \cellcolor{white!38}0.6  & \cellcolor{white!48}0.76 & \cellcolor{white!58}0.82 & \cellcolor{white!58}0.82 
  & \cellcolor{white!32}0.53 & \cellcolor{white!55}0.79 & \cellcolor{white!65}0.84 & \cellcolor{white!65}0.84 
  & \cellcolor{white!30}0.53 & \cellcolor{white!38}0.71 & \cellcolor{white!45}0.77 & \cellcolor{white!45}0.77 \\

\midrule
\multicolumn{17}{c}{\makecell{\textbf{SMP: Decay-Constant ($\lambda$)}\\ \textbf{(fixed $k$=10; $P_{\text{SMP}}$=0.8)}}} \\
\midrule
\textbf{0.3} 
  & \cellcolor{white!38}0.6  & \cellcolor{white!50}0.78 & \cellcolor{white!60}0.82 & \cellcolor{white!60}0.82 
  & \cellcolor{white!45}\textbf{0.65} & \cellcolor{white!52}\textbf{0.79} & \cellcolor{white!65}\textbf{0.86} & \cellcolor{white!65}\textbf{0.86} 
  & \cellcolor{white!35}0.54 & \cellcolor{white!48}0.75 & \cellcolor{white!58}0.79 & \cellcolor{white!58}0.79 
  & \cellcolor{white!35}0.56 & \cellcolor{white!42}0.73 & \cellcolor{white!50}0.78 & \cellcolor{white!50}0.78 \\

0.8 
  & \cellcolor{white!35}\textbf{0.61} & \cellcolor{white!48}\textbf{0.76} & \cellcolor{white!58}\textbf{0.81} & \cellcolor{white!58}\textbf{0.81} 
  & \cellcolor{white!38}0.59 & \cellcolor{white!48}0.73 & \cellcolor{white!58}0.83 & \cellcolor{white!58}0.83 
  & \cellcolor{white!30}0.54 & \cellcolor{white!45}0.72 & \cellcolor{white!55}0.78 & \cellcolor{white!55}0.78 
  & \cellcolor{white!32}0.55 & \cellcolor{white!40}0.74 & \cellcolor{white!48}0.78 & \cellcolor{white!48}0.78 \\

1.0 
  & \cellcolor{white!30}0.58 & \cellcolor{white!42}0.72 & \cellcolor{white!52}0.79 & \cellcolor{white!52}0.79 
  & \cellcolor{white!35}\textbf{0.59} & \cellcolor{white!48}\textbf{0.75} & \cellcolor{white!58}\textbf{0.85} & \cellcolor{white!58}\textbf{0.85} 
  & \cellcolor{white!28}0.53 & \cellcolor{white!42}0.72 & \cellcolor{white!50}0.77 & \cellcolor{white!50}0.77 
  & \cellcolor{white!28}0.52 & \cellcolor{white!38}0.7  & \cellcolor{white!45}0.75 & \cellcolor{white!45}0.75 \\

\midrule
\multicolumn{17}{c}{\makecell{\textbf{SMP: Probability ($P_{\text{SMP}}$)}\\ \textbf{(fixed $k$=10; \(\lambda\)=0.5)}}} \\
\midrule
0.5 
  & \cellcolor{white!35}0.53 & \cellcolor{white!50}0.77 & \cellcolor{white!60}0.84 & \cellcolor{white!60}0.84 
  & \cellcolor{white!40}\textbf{0.59} & \cellcolor{white!52}\textbf{0.77} & \cellcolor{white!58}\textbf{0.82} & \cellcolor{white!58}\textbf{0.82} 
  & \cellcolor{white!38}0.58 & \cellcolor{white!50}0.78 & \cellcolor{white!65}0.84 & \cellcolor{white!65}0.84 
  & \cellcolor{white!38}0.58 & \cellcolor{white!42}0.73 & \cellcolor{white!50}0.78 & \cellcolor{white!50}0.78 \\

\textbf{0.8} 
  & \cellcolor{white!38}0.58 & \cellcolor{white!52}0.79 & \cellcolor{white!62}0.86 & \cellcolor{white!62}0.86 
  & \cellcolor{white!45}\textbf{0.62} & \cellcolor{white!55}\textbf{0.79} & \cellcolor{white!65}\textbf{0.86} & \cellcolor{white!65}\textbf{0.86} 
  & \cellcolor{white!42}0.59 & \cellcolor{white!52}0.78 & \cellcolor{white!68}0.85 & \cellcolor{white!68}0.85 
  & \cellcolor{white!42}0.59 & \cellcolor{white!48}0.77 & \cellcolor{white!55}0.83 & \cellcolor{white!55}0.83 \\

1.0 
  & \cellcolor{white!40}0.59 & \cellcolor{white!55}0.81 & \cellcolor{white!65}0.88 & \cellcolor{white!65}0.88 
  & \cellcolor{white!42}0.57 & \cellcolor{white!50}0.75 & \cellcolor{white!60}0.84 & \cellcolor{white!60}0.84 
  & \cellcolor{white!38}0.57 & \cellcolor{white!48}0.76 & \cellcolor{white!65}0.84 & \cellcolor{white!65}0.84 
  & \cellcolor{white!45}\textbf{0.61} & \cellcolor{white!50}\textbf{0.79} & \cellcolor{white!60}\textbf{0.85} & \cellcolor{white!60}\textbf{0.85} \\

\bottomrule
\end{tabular}%
}
\end{center}
\caption{\textbf{Ablation (RQ-2a.) Effect of \peraugy\ hyper-parameters on User-Encoder Accuracy:} All encoder models are \textit{trained-from-scratch} across various hyper-parameters; summarized results are provided in Table~\ref{tab:ablation-comparative-impact}. \textbf{Observation}: \textit{Best performing hyper-parameter values show consistent performance across encoder models}.}
\label{tab:ablations-accuracy}
\end{table*}


==> tables/tab_encoder-main-results-finetuned.tex <==
\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{TrRMIo w/ Title} (\textbf{Fine-tuned})} \\ 
\cmidrule(lr){2-5}
& AUC & MRR & nDCG@5 & nDCG@10 \\ 
\midrule

\multirow{1}{*}{PENS (Original; \textit{tfs})} & 0.47 & 0.7 & 0.78 & 0.78 \\ 
 % & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
% \midrule

\multirow{1}{*}{PENS-SH} & 0.62 & 0.89 & 0.95 & 0.95 \\ 
% \midrule

\multirow{1}{*}{S3} & 0.51	&	0.76	&	0.80	&	0.80 \\

\multirow{1}{*}{SDAInter} & 0.58	&	0.89	&	0.96	&	0.96 \\ 

\midrule

\multirow{1}{*}{LLaMA2(13B)} & 0.42 & 0.67 & 0.74 & 0.74 \\ 
% \midrule

\multirow{1}{*}{Mistral(7B)}  & 0.56 & 0.73 & 0.75 & 0.75 \\ 
% \midrule

\multirow{1}{*}{DeepSeek-R1}  & 0.47 & 0.69 & 0.77 & 0.77 \\ 
 \midrule
 
 \multirow{1}{*}{ \peraugy\ (\textit{tfs})} & 0.57 & 0.75 & 0.84 & 0.84 \\ 
  \multirow{1}{*}{ \peraugy\ } & \textbf{0.76} & \textbf{0.92} & \textbf{0.97} & \textbf{0.97} \\ 
\bottomrule
\end{tabular}
}
\caption{\textbf{Performance of user encoder (\textit{fine-tuned}):} Best performing TrRMIo model \textit{fine-tuned} with all augmented datasets (on PENS), including \peraugy\ (DS+SMP). \textbf{Observation-1:} \textit{When fine-tuned, \peraugy\ consistently outperforms all baseline augmentation methods compared to their respective fine-tuned versions;} \textbf{Observation-2:} \textit{\peraugy\ also shows a significant performance boost when fine-tuned, relative to its own trained-from-scratch version (denoted as \textit{tfs}).}}% \vspace{-7mm}
\label{tab:encoder-main-result-finetuned}
\end{table}



==> tables/tab_encoder-performance-openai.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccccccccccccccccc}
\toprule
\textbf{Aug. Method} 
& \multicolumn{4}{c}{\textbf{NAML}} 
& \multicolumn{4}{c}{\textbf{EBNR}} 
& \multicolumn{4}{c}{\textbf{NRMS}} 
& \multicolumn{4}{c}{\textbf{TrRMIo w/ Title(w/FT)}} \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
& AUC & MRR & NDCG@5 & NDCG@10 
& AUC & MRR & NDCG@5 & NDCG@10 
& AUC & MRR & NDCG@5 & NDCG@10 
& AUC & MRR & NDCG@5 & NDCG@10 \\ 
\midrule
OpenAI (DS)
& \cellcolor{white!50}0.58 
& \cellcolor{white!60}0.79
& \cellcolor{white!70}0.85 
& \cellcolor{white!70}0.85
& \cellcolor{white!40}0.48 
& \cellcolor{white!65}0.74 
& \cellcolor{white!75}0.81 
& \cellcolor{white!75}0.81
& \cellcolor{white!40}0.60 
& \cellcolor{white!65}0.80 
& \cellcolor{white!75}0.85 
& \cellcolor{white!75}0.85
& \cellcolor{white!50}\textbf{0.68}
& \cellcolor{white!55}\textbf{0.86}
& \cellcolor{white!65}\textbf{0.9} 
& \cellcolor{white!65}\textbf{0.9}\\

\textbf{OpenAI DS+SMP }
& \cellcolor{white!50}0.54
& \cellcolor{white!60}0.81 
& \cellcolor{white!70}0.85 
& \cellcolor{white!70}0.85
& \cellcolor{white!45}0.52 
& \cellcolor{white!67}0.78 
& \cellcolor{white!77}0.84 
& \cellcolor{white!77}0.84
& \cellcolor{white!50}0.63 
& \cellcolor{white!60}0.84 
& \cellcolor{white!70}0.89 
& \cellcolor{white!70}0.89
& \cellcolor{white!45}\textbf{0.69} 
& \cellcolor{white!50}\textbf{0.86}
& \cellcolor{white!60}\textbf{0.91} 
& \cellcolor{white!60}\textbf{0.91} \\
\bottomrule
\end{tabular}%
}
\end{center}
\caption{\textbf{User-Encoder Performance (OpenAI (Reddit))}: Effect of Double Shuffling (DS) and DS+SMP operations on OpenAI (Reddit) seed base (SMP hyper-parameters: $k$=10; $\lambda$=0.3; $p_{SMP}$=0.8)}
% \vspace{-8mm}
\label{tab:peraugy_performance-OpenAI}
\end{table*}

==> tables/tab_parametric-comparison-ablations.tex <==
\begin{table*}[h]
    \begin{center}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcc|cc|cc|cc}
        \toprule
       \textbf{Hyperparameter} & \multicolumn{2}{c}{\textbf{AUC}} & \multicolumn{2}{c}{\textbf{MRR}} & \multicolumn{2}{c}{\textbf{nDCG@5}} & \multicolumn{2}{c}{\textbf{nDCG@10}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        & Rel. Win Margin & Abs. Win Margin & Rel. Win Margin & Abs. Win Margin & Rel. Win Margin & Abs. Win Margin & Rel. Win Margin & Abs. Win Margin \\
        \midrule
        Gap      & 0.018 & 0.043 & 0.005 & 0.021 & 0.007 & 0.023 & 0.007 & 0.018 \\
        History  & 0.024 & 0.064 & 0.013 & 0.035 & 0.011 & 0.026 & 0.011 & 0.028 \\
        Context-k & 0.028 & 0.049 & 0.016 & 0.027 & 0.016 & 0.032 & 0.016 & 0.032 \\
        \(\lambda\)   & 0.019 & 0.034 & 0.023 & 0.047 & 0.010 & 0.029 & 0.010 & 0.029 \\
        Prob     & 0.019 & 0.040 & 0.018 & 0.039 & 0.023 & 0.035 & 0.018 & 0.040 \\
        \bottomrule
    \end{tabular}}
    \end{center}
\caption{\textbf{Ablation: Comparative Impact of Hyper-parameters of \peraugy} ... }
\label{tab:performance_metrics}
\end{table*}




